Reddit Entity Linking Dataset

We introduce and make publicly available an entity linking dataset from Reddit that contains 17,316 linked entities, each annotated by three human annotators and then grouped into Gold, Silver, and Bronze to indicate inter-annotator agreement. We analyze the different errors and disagreements made by annotators and suggest three types of corrections to the raw data. Finally, we tested existing entity linking models that are trained and tuned on text from non-social media datasets. We find that, although these existing entity linking models perform very well on their original datasets, they perform poorly on this social media dataset. We also show that the majority of these errors can be attributed to poor performance on the mention detection subtask. These results indicate the need for better entity linking models that can be applied to the enormous amount of social media text.

==> notes.tex <==
\subsection{Notes}
Stuff to include in the paper/ TODO list of things for it.
 highlight how conversations could provide a larger context for resolution.


Design Challenges for Entity Linking Paper Evaluating Entity Linking: An Analysis of Current Benchmark Datasets and a Roadmap for Doing a Better Job

both of these papers discuss how the problem of entity linking is often not well defined. They also mention how there is a broad difference and understanding of the annotation guidelines. Doing an analysis based on some of the factors they mentioned might be interested. need to also cite them and discuss the points they bring up for our collection.

Examples in data to highlight

playboy playmate example in bronze comment annotations.

playmate meaning a child's friend to play with versus this context.

murder of Saudi dissident journalist Khashoggi - bronze submission

bronze submission - ecuador's embassy


More thourough evaluation of this stuff in the evaluation section. Compare to other datasets that have been released.



==> tables/error_analysis.tex <==
\begin{tabular}{c cc}
\toprule
\textbf{Model} & \textbf{Linking Errors} & \textbf{Mention Errors} \\
\midrule
\textbf{NER + Prior} & 0 & 0 \\
\textbf{NER + Query} & 0 & 0 \\
\textbf{End-to-End} & 0 & 0 \\
\textbf{REL} & 0 & 0 \\
\bottomrule
\end{tabular}

==> tables/new_table-5.tex <==
%\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ll rrr c rrrrrrrr@{}} % {l r||c c c c | c c c c  c c}
\toprule
&  \multirow{2}{*}{\textbf{Model}}   & \multicolumn{3}{c}{\textbf{Reddit Dataset}} & ~ & \multicolumn{8}{c}{\textbf{Other Datasets}} \\ 
 \cmidrule{3-5} \cmidrule{7-14} 
&   & \textbf{Gold} & \textbf{Silver}  & \textbf{Comb.} && \textbf{AI-Trn} & \textbf{AI-A}& \textbf{AI-B} &	\textbf{MSN} &	\textbf{AQNT}	& \textbf{ClueW}& \textbf{WIKI} & \textbf{ACE} \\ \midrule
\multirow{7}{*}{\rotatebox[]{90}{\textbf{$F_1$}}} & \textbf{Query}      &    0.89  &    0.78   & 0.81 && 0.60 & 0.55 & 0.57 & 0.69 & 0.81 & 0.57 & 0.58 & 0.71      \\ 
 & \textbf{Prior}      & 0.78 &  0.66  & 0.70 && 0.74 & 0.71 & 0.69 & 0.76 & 0.83 & 0.67 & 0.64 & 0.84 \\
 & \textbf{Deep-ED}   &   0.80   &    0.71     & 0.74 && 0.87 & 0.87 & 0.88 & 0.93 & 0.90 & 0.76 & 0.74 & 0.88  \\
  & orig. Deep-ED &   --   &    --   & -- &&  -- &-- & \textcolor{gray}{0.92} & \textcolor{gray}{0.94} & \textcolor{gray}{0.86} & \textcolor{gray}{0.78} & \textcolor{gray}{0.78} & \textcolor{gray}{0.89}  \\ 
  & \textbf{mulrel-nel} &   0.72   &    0.63   &  0.67 && --  & 0.92 & 0.93 & 0.93 & 0.88 & 0.77 & 0.77 & 0.91 \\
  & \textbf{wnel} &   0.87   &    0.79   &  0.83 && --  & 0.81 & 0.81 & 0.93 & 0.92 & 0.77 & 0.75 & 0.90 \\
 & \textbf{End-2-End} &   0.85   &    0.76   &  0.80 && 0.97  & 0.94 & 0.87 & 0.92 & 0.90 & 0.77 & 0.74 & 0.88  \\ \midrule

\multirow{2}{*}{\rotatebox[]{90}{\textbf{Cov}}} & \textbf{Query}      &    0.98  &    0.92  &    0.94  &&  0.88    & 0.84 & 0.87  & 0.96  &    0.95  &    0.86    & 0.79  & 0.96     \\ 
 & \textbf{Prior}      &   0.95   &    0.85     &   0.87   &&  0.99     &  0.99 & 0.99 &     0.97    &   0.96   &    0.95    &     0.97 & 0.92  
 %& \textbf{Deep-ED }   &   0.999   &    0.999    &     0.999     &   0.999   &    0.999    &     0.999    &   0.999   &    0.999    &     0.999 & 0.999  \\
 %& \textbf{End-2-End} &   0.999   &    0.999    &     0.999     &   0.999   &    0.999    &     0.999    &   0.999   &    0.999    &     0.999 & 0.999    
 \\ \midrule
\multirow{2}{*}{\rotatebox[]{90}{\textbf{Rank}}} & \textbf{Query}      &    1.33  &    1.52   &    1.45  &&  2.02     & 2.23 & 2.35 & 1.84  &    1.57  &    2.62    & 2.11  & 2.05     \\ 
 & \textbf{Prior}      &    1.26  &    1.40  &   1.36  && 2.40 & 2.79 & 2.63   & 2.17  &    1.68  &    3.18    & 3.86  & 2.11    \\
 %& \textbf{Deep-ED }   &    0.98  &    0.92    & 0.70 &    0.79  &    0.87    & 0.96  &    0.95  &    0.86    & 0.79  & 0.96      \\
 %& \textbf{End-2-End}&    0.98  &    0.92    & 0.70 &    0.79  &    0.87    & 0.96  &    0.95  &    0.86    & 0.79  & 0.96       \\ 
\bottomrule
\end{tabular}
%}

==> tables/new_table-6.tex <==

%\resizebox{\textwidth}{!}{
{\small
\begin{tabular}{@{}ll r c rrrrrrrr@{}} %{l r|c c c c | c c c c  c c}

\toprule
    & \multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Reddit}} & ~ & \multicolumn{8}{c}{\textbf{Other Datasets}} \\ 
    \cmidrule{3-3} \cmidrule{5-11}
&  & \textbf{Comb.} && \textbf{AI-Trn} & \textbf{AI-A}& \textbf{AI-B}  &	\textbf{MSN} &	\textbf{AQNT}	& \textbf{ClueW}& \textbf{WIKI} & \textbf{ACE} \\ \midrule
 \multirow{3}{*}{\rotatebox[]{90}{\textbf{Recall}}} & \textbf{NER + Query}       & 0.24 && 0.46 & 0.41 & 0.42 & 0.52 & 0.34 & 0.39 & 0.28 & 0.57\\
 & \textbf{NER + Prior}      & 0.22 && 0.56 & 0.54 & 0.50 & 0.56 & 0.35 & 0.46 & 0.32 & 0.68  \\
 & \textbf{End-2-End}   & 0.36  && 0.95 & 0.90 & 0.84 & 0.76 & 0.43 & 0.49 & 0.43 & 0.69 \\
 & \textbf{REL}   & 0.00  && 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 \bottomrule
\end{tabular}
}
%}



%\begin{tabular}{@{}ll rrr c rrrrrrrr@{}} %{l r|c c c c | c c c c  c c}

%\toprule
%    & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Reddit Dataset}} & ~ & \multicolumn{8}{c}{\textbf{Other Datasets}} \\ 
%    \cmidrule{3-5} \cmidrule{7-14}
%&  & \textbf{Gold} & \textbf{Silver}  & \textbf{Comb.} && \textbf{AI-Trn} & \textbf{AI-A}& \textbf{AI-B}  &	\textbf{MSN} &	\textbf{AQNT}	& \textbf{ClueW}& \textbf{WIKI} & \textbf{ACE} \\ \midrule
% \multirow{3}{*}{\rotatebox[]{90}{\textbf{Recall}}} & \textbf{NER + Query}       &   0.32   &    0.17   & 0.24 && 0.46 & 0.41 & 0.42 & 0.52 & 0.34 & 0.39 & 0.28 & 0.57\\
% & \textbf{NER + Prior}      &   0.30   &    0.17  & 0.22 && 0.56 & 0.54 & 0.50 & 0.56 & 0.35 & 0.46 & 0.32 & 0.68  \\
% & \textbf{End-2-End}   &   0.40   &    0.33  & 0.36  && 0.95 & 0.90 & 0.84 & 0.76 & 0.43 & 0.49 & 0.43 & 0.69 \\
% & \textbf{REL} &   0.00   &    0.00  & 0.00  && 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
% \bottomrule
%\end{tabular}

==> tables/table-1.tex <==
\begin{tabular}{r|r|r} % {r|l|l}
    \textbf{Subreddit} & \textbf{Posts} & \textbf{Comments} \\ \hline
    r/movies     & 67 & 143 \\ 
    r/worldnews     & 158 & 315 \\ 
    r/gaming     & 30 & 63 \\ 
    r/news     & 84 & 163 \\ 
    r/politics     & 71 & 145 \\ 
    r/explainlikeimfive     & 49 & 90 \\ 
    r/sports     & 72 & 148 \\ 
    r/science     & 47 & 91 \\ 
    r/Economics     & 41 & 85 \\ \hline
    Total & 619 & 1,243
\end{tabular}


==> tables/table-5.tex <==
\begin{tabular}{@{}l r r r r r  r r r r  r r@{}} % {l r||c c c c | c c c c  c c}
\toprule
&     & \multicolumn{4}{c}{\textbf{Reddit Annotation Dataset}} & \multicolumn{6}{c}{\textbf{Other Datasets}} \\ 
 \cmidrule{3-7} \cmidrule{8-12} 
& \textbf{Model}    & \textbf{Gold} & \textbf{Silver} & \textbf{Bronze}  & \textbf{All} & \textbf{AIDA}  &	\textbf{MSNBC} &	\textbf{AQNT}	& \textbf{ClueW}& \textbf{WIKI} & \textbf{ACE} \\ \hline
\multirow{4}{*}{\rotatebox[]{90}{\textbf{$F_1$}}} & \textbf{Query}      &    0.89  &    0.78    & 0.51 & 0.62 & 0.59 & 0.69 & 0.81 & 0.57 & 0.58 & 0.71      \\ 
 & \textbf{Prior}      &   0.78   &    0.66    &    0.40  & 0.51 & 0.71 & 0.76 & 0.83 & 0.67 & 0.64 & 0.84 \\
 & \textbf{Deep-ED}   &   0.82   &    0.72    &    0.45  & 0.56 & 0.87 & 0.93 & 0.90 & 0.76 & 0.74 & 0.88  \\
  & orig. Deep-ED &   --   &    --    &  --   & -- &  \textcolor{gray}{0.92} & \textcolor{gray}{0.94} & \textcolor{gray}{0.86} & \textcolor{gray}{0.78} & \textcolor{gray}{0.78} & \textcolor{gray}{0.89}  \\ 
 & \textbf{End-2-End} &   0.85   &    0.76    &  0.54   & 0.65 &  0.94 & 0.92 & 0.90 & 0.77 & 0.74 & 0.88  \\ \midrule

\multirow{2}{*}{\rotatebox[]{90}{\textbf{Cov}}} & \textbf{Query}      &    0.98  &    0.92    & 0.70 &    0.79  &    0.87    & 0.96  &    0.95  &    0.86    & 0.79  & 0.96     \\ 
 & \textbf{Prior}      &   0.95   &    0.85    &     0.63     &   0.72   &    1.00    &     0.97    &   0.96   &    0.95    &     0.97 & 0.92  
 %& \textbf{Deep-ED }   &   0.999   &    0.999    &     0.999     &   0.999   &    0.999    &     0.999    &   0.999   &    0.999    &     0.999 & 0.999  \\
 %& \textbf{End-2-End} &   0.999   &    0.999    &     0.999     &   0.999   &    0.999    &     0.999    &   0.999   &    0.999    &     0.999 & 0.999    
 \\ \midrule
\multirow{2}{*}{\rotatebox[]{90}{\textbf{Rank}}} & \textbf{Query}      &    1.33  &    1.52    & 1.79  &    1.67  &    2.11    & 1.84  &    1.57  &    2.62    & 2.11  & 2.05     \\ 
 & \textbf{Prior}      &    1.26  &    1.40    & 1.96 &    1.74  &    2.63    & 2.17  &    1.68  &    3.18    & 3.86  & 2.11    \\
 %& \textbf{Deep-ED }   &    0.98  &    0.92    & 0.70 &    0.79  &    0.87    & 0.96  &    0.95  &    0.86    & 0.79  & 0.96      \\
 %& \textbf{End-2-End}&    0.98  &    0.92    & 0.70 &    0.79  &    0.87    & 0.96  &    0.95  &    0.86    & 0.79  & 0.96       \\ 
\bottomrule
\end{tabular}

==> tables/table-6.tex <==
\begin{tabular}{@{}l r r r r r  r r r r  r r@{}} %{l r|c c c c | c c c c  c c}
\toprule
    & & \multicolumn{4}{c}{\textbf{Reddit Annotation Dataset}} & \multicolumn{6}{c}{\textbf{Other Datasets}} \\ 
& \textbf{Model}    & \textbf{Gold} & \textbf{Silver} & \textbf{Bronze}  & \textbf{All} & \textbf{AIDA}  &	\textbf{MSNBC} &	\textbf{AQNT}	& \textbf{ClueW}& \textbf{WIKI} & \textbf{ACE} \\ \midrule
 \multirow{3}{*}{\rotatebox[]{90}{\textbf{Recall}}} & \textbf{NER + Query}       &   0.99   &    0.99    &    0.99  & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 \\
 & \textbf{NER + Prior}      &   0.99   &    0.99    &    0.99  & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 & 0.99 \\
 & \textbf{End-2-End}   &   0.35   &    0.30    &    0.20  & 0.24  & 0.84 & 0.76 & 0.43 & 0.49 & 0.43 & 0.69 \\
 \bottomrule
\end{tabular}

==> tables/top_entities_names.tex <==
\begin{table*}[t]
\centering
\begin{tabularx}{\linewidth}{|l|l|X|}
\hline
Entity & Num. Occurences & Unique Mentions \\ \hline
\textsc{Donald_Trump}       &           87      &    President Trump, Trump, trump, President, trumpian, Donald Trump, Tump, US President Donald Trump, Trump's, 45, his             \\ \hline
United States       &        50         &    U.S., US, American, USA, U.S, America's, United States, America             \\ \hline
Film       &         36        &      Films, films, Movie, movie, FILMS, mocie, movies, Movies, Film, film           \\ \hline
China       &         30        &      china, Chinese, China           \\ \hline
Russia       &          26       &      Russia, Russian, Russians           \\ \hline
Human       &       17          &     human race, Humans, human being, human, Humanity, humans            \\ \hline
Germany & 15 & Germany, germany \\ \hline
Republican Party (US)       &       15          & Republicans, GOP, red, Republican Party                \\ \hline
Research       &         14        &   Researchers, research, researcher, Research, researchers              \\ \hline
Scientist & 14 & scientists, Scientists, scientist \\ \hline
\end{tabularx}
\caption{Top 10 entities from the gold and silver annotations of the dataset. For each entity a list of the mention texts that they were annotated with are shown.}
\label{top_entities_names}
\end{table*}
